Understanding and Modeling Passive-Negative Feedback for Short-video Sequential Recommendation

Sequential recommendation is one of the most important tasks in recommender systems, which aims to recommend the next interacted item with historical behaviors as input. Traditional sequential recommendation always mainly considers the collected positive feedback such as click, purchase, etc. However, in short-video platforms such as TikTok, video viewing behavior may not always represent positive feedback. Specifically, the videos are played automatically, and users passively receive the recommended videos. In this new scenario, users passively express negative feedback by skipping over videos they do not like, which provides valuable information about their preferences. Different from the negative feedback studied in traditional recommender systems, this passive-negative feedback can reflect users' interests and serve as an important supervision signal in extracting users' preferences. Therefore, it is essential to carefully design and utilize it in this novel recommendation scenario. In this work, we first conduct analyses based on a large-scale real-world short-video behavior dataset and illustrate the significance of leveraging passive feedback. We then propose a novel method that deploys the sub-interest encoder, which incorporates positive feedback and passive-negative feedback as supervision signals to learn the user's current active sub-interest. Moreover, we introduce an adaptive fusion layer to integrate various sub-interests effectively. To enhance the robustness of our model, we then introduce a multi-task learning module to simultaneously optimize two kinds of feedback -- passive-negative feedback and traditional randomly-sampled negative feedback. The experiments on two large-scale datasets verify that the proposed method can significantly outperform state-of-the-art approaches. The code is released at https://github.com/tsinghua-fib-lab/RecSys2023-SINE.

==> 5.conclusion.tex <==
\section{Conclusion and Future Work}\label{sec::conclusion}

In this work, we approach a new problem in sequential recommendation systems: understanding and modeling of users' passive-negative feedback in short-video recommendation.
We first use the data analysis on large-scale real-world data to demonstrate 1) it is important,  2) it is challenging, and 3) why it is challenging to utilize passive-negative feedback in sequential recommenders.
\revise{The results show that the passive-negative feedback is similar to the observed positive feedback in video category and thus the intuitive manner of treating it as negative sample does not work well.}
Motivated by the data analysis, we propose a method with a sub-interest extractor, in which the passive-negative feedback can be modeled as the mismatch of specific sub-interests.
The performance comparison shows the best performance of our proposed SINE method.
The further results extensively demonstrate the effectiveness of SINE's different components, and the results correspond well to the earlier data analysis.

As for the future work, we first plan to deploy the proposed SINE model to the real-world online recommendation engine, and evaluate the recommendation performance compared with other methods through the A/B tests. We also plan to collect other kinds of explicit positive feedback, such as like behavior, sharing behavior, etc., to enhance the study of negative feedback in recommender systems, which can motivate us to further improve the model design.






\begin{acks}
This work is partially supported by the National Key Research and Development Program of China under 2022YFB3104702, and the National Natural Science Foundation of China under 62272262, 61972223, U1936217, and U20B2060.
\end{acks}

==> 6.acknowledgements.tex <==
\section{Acknowledgements}\label{sec::acknowledgements}
This work is partially supported by the National Key Research and Development Program of China under 2022YFB3104702, and the National Natural Science Foundation of China under 62272262, 61972223, U1936217, and U20B2060.
